Understanding Cyber Threats Against the Universities, Colleges, and Schools

Universities hold and process a vast amount of valuable user and research data. This makes them a prime target for cyber criminals. Additionally, universities and other educational settings, such as schools and college IT systems, have become a prime target for some of their own students -- often motivated by an opportunity to cause damage to networks and websites, and/or improve their grades. This paper provides a focused assessment of the current cyber security threat to universities, colleges, and schools (`the education sector') worldwide, providing chronological sequencing of attacks and highlighting the insider threat posed by students. Fifty-eight attacks were identified, with ransomware being the most common type of external attack, and hacking motivated by personal gain showing as the most common form of internal attack. Students, who have become a significant internal threat by either aiding or carrying out attacks are not a homogeneous group, as students may be motivated by different factors, therefore calling for targeted responses. Furthermore, the education sector is increasingly reliant on third party IT service providers meaning attacks on third parties can impact the university and its users. There is very little research analysing this problem, even less research analysing the problem in the context of schools. Hence this paper provides one of the first known assessment of the cyber attacks against the education sector, focusing on insider threat posed by students and offering recommendations for mitigating wider cyber threats.

==> references.tex <==
@misc{NCS2022,
  title        ="National Cyber Strategy 2022. Pioneering a cyber future with
the whole of the UK",
  author       = "{HM Government}",
  howpublished = "\url{https://assets.publishing.service.gov.uk/government/uploads/system/uploads/attachment_data/file/1053023/national-cyber-strategy-amend.pdf}",
  year         = 2022,
  note         = "Accessed: 2023-05-19"
}

@misc{NCSC2021,
  title        ="NCSC Annual Review 2021",
  author       = "{NCSC}",
  howpublished = "\url{https://www.ncsc.gov.uk/collection/ncsc-annual-review-2021}",
  year         = 2021,
  note         = "Accessed: 2023-05-19"
}

@misc{netscout2022,
  title        ="DDoS Threat Intelligence Report: Unveiling the New Threat Landscape",
  author       = "{netscout}",
  howpublished = "\url{https://www.netscout.com/threatreport/ddos-threat-intelligence-report/}",
  year         = 2022,
  note         = "Accessed: 2023-05-19"
}

@misc{NCSCalert,
  title        ="Further ransomware attacks on the UK education sector by cyber criminals. Alert, version 2.2",
  author       = "{NCSC}",
  publisher = Crown Copyright
  howpublished = "\url{https://www.ncsc.gov.uk/files/NCSC-Alert-further-ransomware-attacks-UK-education-sector-20210604.pdf}",
  year         = 2021,
  note         = "Accessed: 2023-05-19"
}

@article{almansoori,
  author   = "Almansoori A., Al-Emran M., Shaalan K.",
  title    = "Exploring the Frontiers of Cybersecurity Behavior: A Systematic Review of Studies and Theories",
  journal  = "Applied Sciences",
  year     = 2023,
  volume   = "13",
  number   = "9",
  pages    = "5700",
}

Almansoori A, Al-Emran M, Shaalan K. Exploring the Frontiers of Cybersecurity Behavior: A Systematic Review of Studies and Theories. Applied Sciences. 2023 May 5;13(9):5700.

@article{xu,
  author   = "Almansoori A., Al-Emran M., Shaalan K.",
  title    = "Dual process models of persuasion",
  journal  = "The international encyclopedia of media effects",
  year     = 2017,
  %volume   = "13",
  %number   = "9",
  pages    = "1-3",
}

Xu Q. Dual process models of persuasion. The international encyclopedia of media effects. 2017 Mar 29:1-3.

@article{pinillos,
  author   = "Pinillos, N.Á., Smith, N., Nair, G.S., Marchetto, P., and Mun, C.",
  title    = "Philosophy's New Challenge:
Experiments and Intentional Action",
  journal  = "Mind and Language",
  year     = 2017,
  volume   = "26",
  number   = "1",
  pages    = "115-139",
}

Pinillos, N.Á., Smith, N., Nair, G.S., Marchetto, P., and Mun, C. 2011. “Philosophy's New Challenge:
Experiments and Intentional Action,” Mind and Language (26:1), pp 115-139.

@misc{button2009,
  title        = "Fraud typologies and victims of fraud: literature review",
  author       = "{Button M., Lewis C., Tapley J.}",
  %howpublished = "\url{}",
  publisher = "National Fraud Authority",
  address      = "London",
  year         = "2009",
  note         = "Accessed: 2023-05-19"
}

@article{norris2019,
  author   = "Norris, G., Brookes, A. & Dowell, D.",
  title    = "The Psychology of Internet Fraud Victimisation: a Systematic Review",
  journal  = "J Police Crim Psych",
  year     = 2019,
  volume   = "34",
  %number   = "",
  pages    = "231-245",
}

Norris, G., Brookes, A. & Dowell, D. The Psychology of Internet Fraud Victimisation: a Systematic Review. J Police Crim Psych 34, 231–245 (2019). https://doi.org/10.1007/s11896-019-09334-5

**********
@article{bongiovanni,
  author   = "Bongiovanni, I.",
  title    = "The least secure places in the universe? A systematic literature review on information security management in higher education",
  journal  = "Comput Secur",
  year     = 2019,
  volume   = "86",
  %number   = "6",
  pages    = "350-7",
}

@incollection{singar,
  author    = "Singar, A.V. and Akhilesh, K.B.",
  editor    = "Akhilesh, K. and Möller, D.",
  title     = "Role of Cyber-security in Higher Education,” in Smart Technologies",
  booktitle = "Smart Technologies",
  year      = 2020,
  publisher = "Springer",
  address   = "Singapore",
  pages     = "249–264"
}

@misc{NCSC,
  title        = "The cyber threat to Universities. Assessing the cyber security threat to UK Universities",
  author       = "{NCSC}",
  howpublished = "\url{https://www.ncsc.gov.uk/report/the-cyber-threat-to-universities}",
  year         = 2019,
  note         = "Accessed: 2022-12-28"
}

@article{Alexei,
  author   = "Alexei, L.A.",
  title    = "Network Security Threats to Higher Education Institutions",
  journal  = "Central and Eastern European eDem and eGov Days",
  year     = 2021,
  volume   = "341",
  %number   = "6",
  pages    = " 323–333",
}

@inproceedings{Burov,
  author    = "Burov, O. and Lytvynova, S. and Lavrov, E. and Krylova-Grek, Y. and Orliyk, O. and Petrenko, S. and Shevchenko, S. and Tkachenko, O.M.",
  title     = "Cybersecurity in educational networks,” in Advances in Intelligent Systems and Computing",
  booktitle = "International Conference on Intelligent Human Systems Integration",
  %series    = "NordiCHI",
  year      = 2020,
  pages     = "359-364",
  publisher = "Springer",
  address   = "Cham"
}

@article{Aldawood,
  author   = "Aldawood, H. and Skinner, G.",
  title    = "Reviewing cyber security social engineering training and awareness programs-pitfalls and ongoing issues",
  journal  = "Future Internet",
  year     = 2019,
  volume   = "11",
  number   = "3",
  pages    = "73",
}

@misc{Redscan,
  title        = "The state of cyber security across UK universities: An analysis of Freedom of Information requests",
  author       = "{Redscan}",
  howpublished = "\url{https://www.redscan.com/media/The-state-of- cyber-security-across-UK-universities-Redscan-report.pdf}",
  publisher = {Redscan Cyber Security Limited},
  address      = "London",
  year         = 2020,
  note         = "Accessed: 2020-12-09"
}

@techreport{Chapman,
  title       = "How Safe Is Your Data? Cyber-Security In Higher Education",
  author      = "Chapman, J.",
  institution = "Higher Education Policy Institute",
  address     = "Oxford, UK",
  %number      = "DOE-SLC-6903-1",
  year        = 2019,
  volume   = "12",
  pages    = "1-6"
}

@article{Lagazio,
  author   = "Lagazio, M. and Sherif, N. and Cushman, M.",
  title    = "A multi-level approach to understanding the impact of cyber crime on the financial sector",
  journal  = "Comput Secur",
  year     = 2014,
  volume   = "45",
  %number   = "3",
  pages    = "58-74",
}

@article{Lallie,
  author   = "Lallie, H.S. and Shepherd, L.A. and Nurse, J.R. and, Erola, A. and Epiphaniou, G. and Maple, C. and Bellekens, X.",
  title    = "Cyber security in the age of COVID-19: A timeline and analysis of cyber-crime and cyber-attacks during the pandemic",
  journal = "Computers & Security",
  year     = 2021,
  volume   = "105",
  %number   = "3",
  pages    = "102248",
}

@article{Chng,
  author   = "Chng, S. and Lu, H.Y. and Kumar, A. and Yau, D.",
  title    = "Hacker types, motivations and strategies: A comprehensive framework",
  journal = "Computers in Human Behavior Reports",
  year     = 2022,
  volume   = "5",
  %number   = "3",
  pages    = "100167",
}

@article{Rogers,
  author   = "Rogers, M.K.",
  title    = "A two-dimensional circumplex approach to the development of a hacker taxonomy",
  journal = "Digit Investig",
  year     = 2006,
  volume   = "3",
  number   = "2",
  pages    = "97-102",
}

@misc{NCSC2,
  title        = "Alert: Further ransomware attacks on the UK education sector by cyber criminals",
  author       = "{NCSC}",
  howpublished = "\url{https://www.ncsc.gov.uk/news/alert-targeted-ransomware-attacks-on-uk-education-sector}",
  year         = 2021,
  month   = June,
  day = 4
  note         = "Accessed: 2022-12-26"
}

@misc{DfE,
  title        = "Meeting digital and technology standards in schools and colleges",
  author       = "{Department for Education}",
  howpublished = "\url{https://www.gov.uk/guidance/meeting-digital-and-technology-standards-in-schools-and-colleges/cyber-security-standards-for-schools-and-colleges}",
  year         = 2022,
  note         = "Accessed: 2022-12-28"
}

@misc{CISA,
  title        = "Insider Threat Mitigation Guide",
  author       = "{Cybersecurity and Infrastructure Security Agency}",
  howpublished = "\url{https://www.cisa.gov/sites/default/files/publications/Insider%20Threat%20Mitigation%20Guide_Final_508.pdf}",
  year         = 2020,
  note         = "Accessed: 2022-12-28"
}

@incollection{Bada,
  author    = "Bada, M. and Nurse, J.R.C.",
  editor    = "Benson, V. and Mcalaney, J.",
  title     = "The social and psychological impact of cyberattacks",
  booktitle = "Emerging Cyber Threats and Cognitive Vulnerabilities",
  year      = 2020,
  publisher = "Academic Press",
  %address   = "New York, NY",
  pages     = "73-92"
}
```
@article{Kemp,
  author   = "Kemp, S. and Buil-Gil, D. and Miró-Llinares, F. and Lord, N.",
  title    = "When do businesses report cybercrime? Findings from a UK study",
  journal = "Criminology and Criminal Justice",
  year     = 2021,
  volume   = "0",
  number   = "0",
  pages    = "17488958211062359",
}

@misc{Hellfire,
  title        = "Hacker collective leaks one million records, vows ’hellfire",
  author       = "{Infosecurity Magazine}",
  howpublished = "\url{https://www.infosecurity-magazine.com/ news/hacker-collective-leaks-one-million-records-vows/}",
  year         = 2012,
  note         = "Accessed: 2021-03-15"
}

@misc{NFIB,
  title        = "Cyber crime trends, 2021",
  %author       = "{Infosecurity Magazine}",
  howpublished = "\url{https://data.actionfraud. police.uk/cms/wp-content/uploads/2021/07/CYBER-Dashboard- Assessment-20-21.pdf}",
  %year         = 2012,
  note         = "Accessed: 2021-09-15"
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
[1]	I. Bongiovanni, “The least secure places in the universe? A systematic literature review on information security management in higher education,” Comput Secur, vol. 86, 2019, doi: 10.1016/j.cose.2019.07.003.
[2]	A. v. Singar and K. B. Akhilesh, “Role of Cyber-security in Higher Education,” in Smart Technologies, 2020. doi: 10.1007/978-981-13-7139-4_19.
[3]	NCSC, “The cyber threat to Universities. Assessing the cyber security threat to UK Universities,” Sep. 2019. Accessed: Dec. 28, 2022. [Online]. Available: https://www.ncsc.gov.uk/report/the-cyber-threat-to-universities
[4]	A. Arina, “Network Security Threats to Higher Education Institutions,” Central and Eastern European eDem and eGov Days, vol. 341, pp. 323–333, Mar. 2022, doi: 10.24989/ocg.v341.24.
[5]	O. Burov et al., “Cybersecurity in educational networks,” in Advances in Intelligent Systems and Computing, 2020, vol. 1131 AISC. doi: 10.1007/978-3-030-39512-4_56.
[6]	H. Aldawood and G. Skinner, “Reviewing cyber security social engineering training and awareness programs-pitfalls and ongoing issues,” Future Internet, vol. 11, no. 3. 2019. doi: 10.3390/fi11030073.
[7]	Redscan, “The state of cyber security across UK universities: An analysis of Freedom of Information requests,” London, 2020. Accessed: Dec. 09, 2020. [Online]. Available: https://www.redscan.com/media/The-state-of- cyber-security-across-UK-universities-Redscan-report.pdf
[8]	J. Chapman, “How Safe Is Your Data? Cyber-Security In Higher Education,” HEPI Policy note, no. April, 2019.
[9]	M. Lagazio, N. Sherif, and M. Cushman, “A multi-level approach to understanding the impact of cyber crime on the financial sector,” Comput Secur, vol. 45, 2014, doi: 10.1016/j.cose.2014.05.006.
[10]	H. S. Lallie et al., “Cyber security in the age of COVID-19: A timeline and analysis of cyber-crime and cyber-attacks during the pandemic,” Comput Secur, vol. 105, 2021, doi: 10.1016/j.cose.2021.102248.
[11]	S. Chng, H. Y. Lu, A. Kumar, and D. Yau, “Hacker types, motivations and strategies: A comprehensive framework,” Computers in Human Behavior Reports, vol. 5. 2022. doi: 10.1016/j.chbr.2022.100167.
[12]	M. K. Rogers, “A two-dimensional circumplex approach to the development of a hacker taxonomy,” Digit Investig, vol. 3, no. 2, 2006, doi: 10.1016/j.diin.2006.03.001.
[13]	NCSC, “Alert: Further ransomware attacks on the UK education sector by cyber criminals,” Mar. 23, 2021. https://www.ncsc.gov.uk/news/alert-targeted-ransomware-attacks-on-uk-education-sector (accessed Dec. 26, 2022).
[14]	Department for Education, “Meeting digital and technology standards in schools and colleges,” Mar. 2022, Accessed: Dec. 28, 2022. [Online]. Available: https://www.gov.uk/guidance/meeting-digital-and-technology-standards-in-schools-and-colleges/cyber-security-standards-for-schools-and-colleges
[15]	M. Bada and J. R. C. Nurse, “The social and psychological impact of cyberattacks,” in Emerging Cyber Threats and Cognitive Vulnerabilities, 2020. doi: 10.1016/b978-0-12-816203-3.00004-6.
[16]	S. Kemp, D. Buil-Gil, F. Miró-Llinares, and N. Lord, “When do businesses report cybercrime? Findings from a UK study,” Criminology and Criminal Justice, 2021, doi: 10.1177/17488958211062359.

